Pretraining Language Models for Diachronic Linguistic Change Discovery

Large language models (LLMs) have shown potential as tools for scientific discovery. This has engendered growing interest in their use in humanistic disciplines, such as historical linguistics and literary studies. These fields often construct arguments on the basis of delineations like genre, or more inflexibly, time period. Although efforts have been made to restrict inference to specific domains via fine-tuning or model editing, we posit that the only true guarantee is domain-restricted pretraining -- typically, a data- and compute-expensive proposition. We show that efficient pretraining techniques can produce useful models over corpora too large for easy manual inspection but too small for "typical" LLM approaches. We employ a novel date-attribution pipeline in order to obtain a temporally-segmented dataset of five 10-million-word slices. We train two corresponding five-model batteries over these corpus segments, efficient pretraining and Llama3-8B parameter efficiently finetuned. We find that the pretrained models are faster to train than the finetuned baselines and that they better respect the historical divisions of our corpus. Emphasizing speed and precision over a-historical comprehensiveness enables a number of novel approaches to hypothesis discovery and testing in our target fields. Taking up diachronic linguistics as a testbed, we show that our method enables the detection of a diverse set of phenomena, including en masse lexical change, non-lexical (grammatical and morphological) change, and word sense introduction/obsolescence. We provide a ready-to-use pipeline that allows extension of our approach to other target fields with only minimal adaptation.

==> tables/blimp_outliers_dora.tex <==
\begin{longtable}{lrrrrr}
 & 1750-1820 & 1820-1850 & 1850-1880 & 1880-1910 & 1910-1940 \\
alias &  &  &  &  &  \\
\endfirsthead
 & 1750-1820 & 1820-1850 & 1850-1880 & 1880-1910 & 1910-1940 \\
alias &  &  &  &  &  \\
\endhead
\multicolumn{6}{r}{Continued on next page} \\
\endfoot
\endlastfoot
 & 0.80 & 0.81 & 0.83 & 0.84 & 0.84 \\
 adjunct island & \bfseries 0.84 & 0.86 & 0.87 & 0.88 & 0.86 \\
 anaphor gender agr & 0.95 & 0.96 & 0.96 & 0.97 & 0.97 \\
 anaphor number agr & 0.99 & 0.99 & \bfseries 1.00 & 0.99 & \bfseries 0.98 \\
 animate subject passive & 0.77 & 0.79 & 0.80 & 0.81 & 0.80 \\
 animate subject trans & 0.87 & 0.88 & 0.89 & 0.90 & 0.89 \\
 causative & 0.73 & 0.75 & 0.79 & 0.79 & 0.78 \\
 complex NP island & 0.60 & 0.60 & 0.62 & 0.58 & 0.62 \\
 coord structure const complex left branch & 0.82 & 0.86 & 0.85 & 0.86 & 0.83 \\
 coord structure const object extraction & 0.88 & 0.84 & 0.88 & 0.85 & 0.83 \\
 det noun agr 1 & 1.00 & 0.99 & 1.00 & 1.00 & 1.00 \\
 det noun agr 2 & 0.99 & 1.00 & 0.99 & 1.00 & 1.00 \\
 det noun agr irrg 1 & 1.00 & 1.00 & 1.00 & 0.99 & 1.00 \\
 det noun agr irrg 2 & 0.99 & \bfseries 0.99 & 0.99 & 0.99 & \bfseries 0.99 \\
 det noun agr with adj 2 & 0.96 & 0.96 & 0.97 & 0.97 & 0.97 \\
 det noun agr with adj irrg 1 & 0.98 & 0.98 & 0.99 & 0.99 & 0.97 \\
 det noun agr with adj irrg 2 & 0.97 & 0.97 & 0.99 & 0.98 & 0.99 \\
 det noun agr with adjective 1 & \bfseries 0.96 & 0.98 & 0.97 & 0.99 & 0.98 \\
 distractor agr relational noun & 0.86 & 0.88 & 0.90 & 0.93 & 0.92 \\
 distractor agr relative clause & 0.77 & 0.79 & 0.79 & 0.86 & 0.83 \\
 drop argument & 0.76 & 0.79 & 0.81 & 0.84 & 0.85 \\
 ellipsis n bar 1 & \bfseries 0.84 & 0.87 & 0.89 & 0.88 & 0.86 \\
 ellipsis n bar 2 & 0.86 & 0.87 & 0.84 & 0.86 & 0.87 \\
 existential there object raising & 0.83 & 0.81 & 0.81 & \bfseries 0.75 & 0.79 \\
 existential there quantifiers 1 & 0.98 & 0.99 & 0.99 & 1.00 & 0.99 \\
 existential there quantifiers 2 & 0.81 & 0.81 & 0.74 & 0.77 & 0.78 \\
 existential there subject raising & 0.90 & 0.91 & 0.93 & 0.94 & 0.92 \\
 expletive it object raising & \bfseries 0.75 & 0.76 & 0.76 & 0.76 & \bfseries 0.76 \\
 inchoative & \bfseries 0.61 & 0.68 & 0.70 & 0.70 & 0.70 \\
 intransitive & 0.79 & 0.82 & 0.86 & 0.87 & 0.87 \\
 irrg past participle adjectives & 0.89 & 0.91 & 0.97 & 0.98 & 0.98 \\
 irrg past participle verbs & 0.85 & 0.83 & 0.90 & 0.94 & 0.94 \\
 irrg plural subject verb agr 1 & 0.96 & 0.95 & 0.96 & 0.96 & 0.97 \\
 irrg plural subject verb agr 2 & 0.91 & 0.94 & 0.96 & 0.97 & 0.96 \\
 left branch island echo question & 0.61 & 0.62 & 0.59 & 0.57 & 0.61 \\
 left branch island simple question & 0.91 & 0.91 & 0.91 & 0.92 & 0.92 \\
 matrix question npi licensor present & 0.54 & 0.54 & 0.59 & 0.65 & 0.63 \\
 npi present 1 & \bfseries 0.39 & 0.53 & 0.53 & 0.57 & 0.55 \\
 npi present 2 & 0.57 & 0.60 & 0.63 & 0.64 & 0.65 \\
 only npi licensor present & 0.92 & 0.96 & 0.98 & 1.00 & 0.99 \\
 only npi scope & 0.67 & 0.73 & 0.78 & 0.77 & 0.72 \\
 passive 1 & 0.85 & 0.85 & 0.88 & 0.89 & 0.88 \\
 passive 2 & 0.88 & 0.88 & 0.90 & 0.91 & 0.90 \\
 principle A c command & 0.76 & 0.77 & 0.83 & 0.85 & 0.83 \\
 principle A case 1 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 principle A case 2 & 0.79 & 0.84 & 0.88 & 0.92 & 0.91 \\
 principle A domain 1 & \bfseries 0.99 & 0.99 & 0.99 & 0.99 & 0.99 \\
 principle A domain 2 & 0.81 & 0.82 & 0.86 & 0.85 & 0.83 \\
 principle A domain 3 & 0.63 & 0.63 & 0.67 & 0.67 & 0.65 \\
 principle A reconstruction & 0.30 & 0.18 & 0.32 & 0.25 & 0.27 \\
 regular plural subject verb agr 1 & \bfseries 0.95 & 0.97 & 0.99 & 0.98 & 0.97 \\
 regular plural subject verb agr 2 & 0.87 & 0.90 & 0.89 & 0.92 & 0.92 \\
 sentential negation npi licensor present & \bfseries 0.99 & 0.99 & 0.99 & 0.99 & \bfseries 1.00 \\
 sentential negation npi scope & 0.54 & 0.59 & 0.62 & 0.62 & 0.67 \\
 sentential subject island & 0.55 & 0.42 & 0.47 & 0.51 & 0.52 \\
 superlative quantifiers 1 & 0.94 & 0.93 & 0.97 & 0.96 & 0.97 \\
 superlative quantifiers 2 & 0.70 & 0.75 & 0.80 & 0.79 & 0.81 \\
 tough vs raising 1 & 0.52 & 0.56 & 0.62 & 0.67 & 0.66 \\
 tough vs raising 2 & 0.92 & 0.91 & 0.91 & 0.91 & \bfseries 0.90 \\
 transitive & 0.79 & 0.77 & 0.81 & 0.83 & 0.86 \\
 wh island & 0.69 & 0.70 & 0.65 & 0.74 & 0.79 \\
 wh questions object gap & 0.83 & 0.85 & 0.87 & 0.86 & 0.86 \\
 wh questions subject gap & 0.93 & 0.94 & 0.93 & \bfseries 0.94 & 0.93 \\
 wh questions subject gap long distance & 0.87 & 0.89 & 0.87 & 0.89 & 0.86 \\
 wh vs that no gap & 0.94 & 0.95 & 0.97 & 0.96 & 0.95 \\
 wh vs that no gap long distance & 0.95 & 0.94 & 0.97 & 0.96 & 0.97 \\
 wh vs that with gap & \bfseries 0.45 & 0.41 & 0.42 & 0.42 & 0.41 \\
 wh vs that with gap long distance & \bfseries 0.48 & 0.45 & 0.45 & 0.45 & \bfseries 0.41 \\
\end{longtable}


==> tables/blimp_outliers_students.tex <==
\begin{longtable}{lrrrrr}
 & 1750-1820 & 1820-1850 & 1850-1880 & 1880-1910 & 1910-1940 \\
alias &  &  &  &  &  \\
\endfirsthead
 & 1750-1820 & 1820-1850 & 1850-1880 & 1880-1910 & 1910-1940 \\
alias &  &  &  &  &  \\
\endhead
\multicolumn{6}{r}{Continued on next page} \\
\endfoot
\endlastfoot
 & 0.67 & 0.68 & 0.69 & 0.72 & 0.72 \\
 adjunct island & 0.74 & 0.77 & 0.81 & 0.80 & 0.73 \\
 anaphor gender agr & 0.83 & 0.84 & 0.91 & 0.91 & 0.94 \\
 anaphor number agr & 0.96 & 0.94 & 0.99 & 0.98 & 0.99 \\
 animate subject passive & 0.74 & 0.73 & 0.72 & 0.75 & 0.72 \\
 animate subject trans & 0.80 & 0.85 & 0.84 & 0.88 & 0.89 \\
 causative & 0.59 & \bfseries 0.50 & 0.59 & \bfseries 0.61 & 0.60 \\
 complex NP island & 0.59 & 0.53 & 0.47 & 0.51 & 0.49 \\
 coord structure const complex left branch & 0.44 & 0.41 & 0.29 & 0.34 & 0.28 \\
 coord structure const object extraction & 0.74 & 0.75 & 0.77 & 0.72 & 0.79 \\
 det noun agr 1 & 0.95 & 0.96 & 0.97 & 0.96 & 0.97 \\
 det noun agr 2 & 0.94 & 0.95 & 0.96 & 0.97 & \bfseries 0.90 \\
 det noun agr irrg 1 & \bfseries 0.87 & 0.95 & 0.96 & \bfseries 0.99 & 0.95 \\
 det noun agr irrg 2 & 0.92 & 0.90 & 0.96 & 0.96 & 0.94 \\
 det noun agr with adj 2 & \bfseries 0.91 & 0.94 & 0.93 & \bfseries 0.95 & 0.94 \\
 det noun agr with adj irrg 1 & 0.92 & 0.94 & 0.97 & 0.98 & 0.96 \\
 det noun agr with adj irrg 2 & 0.92 & 0.93 & 0.96 & 0.95 & 0.95 \\
 det noun agr with adjective 1 & \bfseries 0.90 & 0.92 & 0.94 & 0.92 & 0.93 \\
 distractor agr relational noun & 0.86 & \bfseries 0.80 & 0.88 & 0.90 & 0.87 \\
 distractor agr relative clause & 0.44 & 0.44 & 0.57 & 0.50 & 0.53 \\
 drop argument & 0.71 & 0.71 & 0.69 & 0.73 & 0.76 \\
 ellipsis n bar 1 & \bfseries 0.64 & 0.71 & 0.74 & \bfseries 0.80 & 0.73 \\
 ellipsis n bar 2 & 0.50 & 0.52 & 0.53 & 0.55 & 0.50 \\
 existential there object raising & 0.79 & 0.81 & 0.79 & 0.76 & 0.74 \\
 existential there quantifiers 1 & \bfseries 0.99 & 1.00 & \bfseries 1.00 & 1.00 & 1.00 \\
 existential there quantifiers 2 & 0.29 & 0.40 & 0.28 & 0.10 & 0.20 \\
 existential there subject raising & 0.77 & 0.85 & 0.83 & 0.88 & 0.81 \\
 expletive it object raising & \bfseries 0.67 & 0.73 & 0.73 & 0.73 & 0.71 \\
 inchoative & \bfseries 0.46 & 0.50 & 0.51 & 0.51 & \bfseries 0.55 \\
 intransitive & 0.64 & 0.66 & 0.70 & 0.72 & 0.75 \\
 irrg past participle adjectives & 0.96 & \bfseries 0.88 & 0.96 & 0.98 & 0.93 \\
 irrg past participle verbs & 0.82 & 0.84 & 0.89 & 0.86 & 0.90 \\
 irrg plural subject verb agr 1 & 0.83 & 0.79 & 0.88 & 0.89 & 0.89 \\
 irrg plural subject verb agr 2 & 0.91 & \bfseries 0.88 & 0.90 & \bfseries 0.93 & 0.90 \\
 left branch island echo question & 0.18 & 0.37 & 0.30 & 0.38 & 0.44 \\
 left branch island simple question & 0.51 & 0.48 & 0.44 & 0.49 & 0.42 \\
 matrix question npi licensor present & \bfseries 0.09 & 0.14 & 0.13 & \bfseries 0.20 & 0.13 \\
 npi present 1 & 0.19 & 0.23 & 0.22 & 0.24 & \bfseries 0.32 \\
 npi present 2 & 0.30 & 0.31 & 0.36 & 0.26 & 0.37 \\
 only npi licensor present & 0.00 & 0.00 & 0.33 & 0.82 & 0.91 \\
 only npi scope & 0.31 & 0.47 & 0.53 & 0.42 & 0.49 \\
 passive 1 & 0.74 & 0.77 & 0.82 & 0.84 & 0.86 \\
 passive 2 & \bfseries 0.73 & 0.80 & 0.81 & 0.82 & \bfseries 0.85 \\
 principle A c command & \bfseries 0.63 & 0.59 & 0.60 & \bfseries 0.56 & 0.59 \\
 principle A case 1 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 principle A case 2 & \bfseries 0.67 & 0.82 & 0.85 & 0.84 & 0.88 \\
 principle A domain 1 & 0.99 & 0.99 & 0.99 & 0.99 & 1.00 \\
 principle A domain 2 & \bfseries 0.66 & 0.72 & 0.75 & \bfseries 0.82 & 0.75 \\
 principle A domain 3 & 0.56 & 0.55 & 0.58 & 0.63 & 0.65 \\
 principle A reconstruction & 0.11 & 0.20 & 0.10 & 0.22 & 0.22 \\
 regular plural subject verb agr 1 & 0.82 & 0.82 & 0.86 & 0.88 & 0.90 \\
 regular plural subject verb agr 2 & 0.83 & 0.78 & 0.80 & 0.86 & 0.86 \\
 sentential negation npi licensor present & 1.00 & 1.00 & \bfseries 0.99 & 1.00 & \bfseries 1.00 \\
 sentential negation npi scope & 0.23 & 0.25 & 0.19 & 0.20 & 0.19 \\
 sentential subject island & 0.43 & 0.38 & 0.35 & 0.37 & 0.41 \\
 superlative quantifiers 1 & 1.00 & 0.97 & 0.91 & 0.92 & 0.94 \\
 superlative quantifiers 2 & 0.78 & 0.59 & 0.55 & 0.86 & 0.62 \\
 tough vs raising 1 & 0.17 & 0.19 & 0.23 & 0.29 & 0.33 \\
 tough vs raising 2 & 0.91 & 0.90 & 0.91 & 0.87 & 0.85 \\
 transitive & 0.64 & 0.66 & 0.68 & 0.68 & \bfseries 0.72 \\
 wh island & 0.76 & 0.64 & 0.67 & 0.70 & 0.80 \\
 wh questions object gap & 0.71 & 0.70 & \bfseries 0.55 & 0.78 & 0.77 \\
 wh questions subject gap & 0.93 & 0.89 & \bfseries 0.85 & 0.89 & 0.91 \\
 wh questions subject gap long distance & 0.86 & \bfseries 0.77 & 0.90 & 0.88 & 0.86 \\
 wh vs that no gap & 0.97 & 0.93 & 0.95 & 0.94 & 0.97 \\
 wh vs that no gap long distance & 0.94 & 0.92 & 0.95 & 0.95 & 0.96 \\
 wh vs that with gap & 0.28 & 0.41 & 0.31 & 0.37 & 0.30 \\
 wh vs that with gap long distance & 0.19 & \bfseries 0.25 & 0.20 & 0.12 & 0.16 \\
\end{longtable}


==> tables/cloze_olympic_permute.tex <==
\begin{tabular}{llrl}
\toprule
model & text & rank & top answer \\
\midrule
babyllama 1910 1940 & She took second in the high dive, earning a silver & NaN &  little \\
babyllama 1910 1940 & She took first in the high dive, earning a silver & NaN &  little \\
babyllama 1910 1940 & He took second in the high dive, earning a silver & NaN &  little \\
babyllama 1910 1940 & He took first in the high dive, earning a silver & NaN &  little \\
babyllama 1910 1940 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & NaN &  little \\
babyllama 1910 1940 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & NaN &  little \\
babyllama 1910 1940 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & 13.000000 &  little \\
babyllama 1910 1940 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & 18.000000 &  little \\
dora 1910 1940 & She took second in the high dive, earning a silver & 3.000000 &  blue \\
dora 1910 1940 & She took first in the high dive, earning a silver & 2.000000 &  blue \\
dora 1910 1940 & He took second in the high dive, earning a silver & 1.000000 &  gold \\
dora 1910 1940 & He took first in the high dive, earning a silver & 1.000000 &  gold \\
dora 1910 1940 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & 0.000000 &  silver \\
dora 1910 1940 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & 3.000000 &  gold \\
dora 1910 1940 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & 0.000000 &  silver \\
dora 1910 1940 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & 2.000000 &  gold \\
babyllama 1820 1850 & She took second in the high dive, earning a silver & NaN &  little \\
babyllama 1820 1850 & She took first in the high dive, earning a silver & NaN &  little \\
babyllama 1820 1850 & He took second in the high dive, earning a silver & NaN &  little \\
babyllama 1820 1850 & He took first in the high dive, earning a silver & NaN &  little \\
babyllama 1820 1850 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & NaN &  certain \\
babyllama 1820 1850 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & NaN &  certain \\
babyllama 1820 1850 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & NaN &  new \\
babyllama 1820 1850 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & NaN &  new \\
dora 1820 1850 & She took second in the high dive, earning a silver & 0.000000 &  silver \\
dora 1820 1850 & She took first in the high dive, earning a silver & 5.000000 &  round \\
dora 1820 1850 & He took second in the high dive, earning a silver & 0.000000 &  silver \\
dora 1820 1850 & He took first in the high dive, earning a silver & 6.000000 &  cheer \\
dora 1820 1850 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & 0.000000 &  silver \\
dora 1820 1850 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & 1.000000 &  gold \\
dora 1820 1850 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & 0.000000 &  silver \\
dora 1820 1850 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & 1.000000 &  gold \\
babyllama 1750 1820 & She took second in the high dive, earning a silver & 41.000000 &  little \\
babyllama 1750 1820 & She took first in the high dive, earning a silver & 43.000000 &  little \\
babyllama 1750 1820 & He took second in the high dive, earning a silver & 41.000000 &  little \\
babyllama 1750 1820 & He took first in the high dive, earning a silver & 43.000000 &  little \\
babyllama 1750 1820 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & NaN &  great \\
babyllama 1750 1820 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & NaN &  great \\
babyllama 1750 1820 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & NaN &  certain \\
babyllama 1750 1820 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & NaN &  little \\
dora 1750 1820 & She took second in the high dive, earning a silver & 1.000000 &  guinea \\
dora 1750 1820 & She took first in the high dive, earning a silver & 2.000000 &  guinea \\
dora 1750 1820 & He took second in the high dive, earning a silver & 1.000000 &  guinea \\
dora 1750 1820 & He took first in the high dive, earning a silver & 2.000000 &  guinea \\
dora 1750 1820 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & 0.000000 &  silver \\
dora 1750 1820 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & 3.000000 &  gold \\
dora 1750 1820 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & 0.000000 &  silver \\
dora 1750 1820 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & 1.000000 &  gold \\
babyllama 1880 1910 & She took second in the high dive, earning a silver & 17.000000 &  little \\
babyllama 1880 1910 & She took first in the high dive, earning a silver & 17.000000 &  little \\
babyllama 1880 1910 & He took second in the high dive, earning a silver & 18.000000 &  little \\
babyllama 1880 1910 & He took first in the high dive, earning a silver & 17.000000 &  little \\
babyllama 1880 1910 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & 23.000000 &  picture \\
babyllama 1880 1910 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & 20.000000 &  picture \\
babyllama 1880 1910 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & 9.000000 &  second \\
babyllama 1880 1910 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & 16.000000 &  second \\
dora 1880 1910 & She took second in the high dive, earning a silver & 1.000000 &  medal \\
dora 1880 1910 & She took first in the high dive, earning a silver & 3.000000 &  medal \\
dora 1880 1910 & He took second in the high dive, earning a silver & 1.000000 &  medal \\
dora 1880 1910 & He took first in the high dive, earning a silver & 2.000000 &  medal \\
dora 1880 1910 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & 0.000000 &  silver \\
dora 1880 1910 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & 1.000000 &  gold \\
dora 1880 1910 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & 0.000000 &  silver \\
dora 1880 1910 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & 2.000000 &  gold \\
babyllama 1850 1880 & She took second in the high dive, earning a silver & 41.000000 &  little \\
babyllama 1850 1880 & She took first in the high dive, earning a silver & 37.000000 &  little \\
babyllama 1850 1880 & He took second in the high dive, earning a silver & 42.000000 &  little \\
babyllama 1850 1880 & He took first in the high dive, earning a silver & 36.000000 &  little \\
babyllama 1850 1880 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & NaN &  good \\
babyllama 1850 1880 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & NaN &  good \\
babyllama 1850 1880 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & 22.000000 &  hundred \\
babyllama 1850 1880 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & 27.000000 &  hundred \\
dora 1850 1880 & She took second in the high dive, earning a silver & 1.000000 &  prize \\
dora 1850 1880 & She took first in the high dive, earning a silver & 2.000000 &  prize \\
dora 1850 1880 & He took second in the high dive, earning a silver & 0.000000 &  silver \\
dora 1850 1880 & He took first in the high dive, earning a silver & 2.000000 &  prize \\
dora 1850 1880 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example second place earns a silver & 0.000000 &  silver \\
dora 1850 1880 & The composition of Olympic medals tie a precious metal to the quality of a finish, for example first place earns a silver & 1.000000 &  gold \\
dora 1850 1880 & In the Olympics, the third place finisher in an event wins a bronze while the second earns a silver & 0.000000 &  silver \\
dora 1850 1880 & In the Olympics, the third place finisher in an event wins a bronze while the first earns a silver & 2.000000 &  gold \\
\bottomrule
\end{tabular}
